Rejuvenating IRS: AoI-based Low Overhead Reconfiguration Design

Intelligent reflective surface (IRS) technologies help mitigate undesirable effects in wireless links by steering the communication signal between transmitters and receivers. IRS elements are configured to adjust the phase of the reflected signal for a user's location and enhance the perceived signal-to-noise ratio (SNR). In this way, an IRS improves the communication link but inevitably introduces more communication overhead. This occurs especially in mobile scenarios, where the user's position must be frequently estimated to re-adjust the IRS elements periodically. Such an operation requires balancing the amount of training versus the data time slots to optimize the communication performance in the link. Aiming to study this balance with the age of information (AoI) framework, we address the question of how often an IRS needs to be updated with the lowest possible overhead and the maximum of freshness of information. We derive the corresponding analytical solution for a mobile scenario, where the transmitter is static and the mobile user (MU) follows a random waypoint mobility model. We provide a closed-form expression for the average peak age of information (PAoI), as a metric to evaluate the impact of the IRS update frequency. As for the performance evaluation, we consider a realistic scenario following the IEEE 802.11ad standard, targeting the mmWave band. Our results reveal that the minimum achievable average PAoI is in the microsecond range and the optimal IRS update period is in the seconds range, causing 9% overhead in the link when the MU moves at a velocity of 1 m/s.

==> acro.tex <==
% Acronyms
\RequirePackage[]{acronym}

%related to metric units
\acrodef{SI}{international system}
\acrodef{CGS}{centimeter-gram-second}
 
%related to computer networks
\acrodef{ICT}{information and communication technology}
\acrodef{IoT}{Internet of Things}
\acrodef{AoI}{age of information}
\acrodef{PAoI}{peak age of information}
\acrodef{CPS}{cyber-physical system}
\acrodef{UAV}{unmanned aerial vehicle}
\acrodef{RWP}{random waypoint}
\acrodef{BS}{base station}
\acrodef{MU}{mobile user}
\acrodef{NLOS}{non-line-of-sight}
\acrodef{LOS}{line-of-sight}
\acrodef{B5G}{beyond fifth generation}
\acrodef{5G}{fifth generation}
\acrodef{6G}{sixth generation}
\acrodef{FC}{fusion node}
\acrodef{IoMT}{internet of mobile things}
\acrodef{OWA}{ordered weighted averaging}
\acrodef{PU}{primary user}
\acrodef{SU}{secondary user}
\acrodef{CSS}{cooperative spectrum sensing}
\acrodef{WSN}{wireless sensor network}
\acrodef{ISM}{industrial, scientific, and medical}
 
 
%related WiFi technologies
\acrodef{AP}{access point}
\acrodef{WuR}{wake-up radio}
\acrodef{CSI}{channel state information}
\acrodef{CIR}{channel impulse response}
\acrodef{ISI}{inter-symbol interference}
\acrodef{Tx}{transmitter}
\acrodef{RF}{radio frequency}
\acrodef{Rx}{receiver}
\acrodef{LTV}{linear time-variant}
\acrodef{BER}{bit error rate}
\acrodef{FER}{frame error rate}
\acrodef{PER}{packet error rate}
\acrodef{PPM}{pulse position modulation}
\acrodef{OOK}{on-off keying}
\acrodef{BPSK}{binary phase shift keying}
\acrodef{PSK}{phase shift keying}
\acrodef{QAM}{quadrature amplitude modulation}
\acrodef{SNR}{signal-to-noise ratio}
\acrodef{RMS}{root mean square}
\acrodef{AWGN}{additive white gaussian noise}
\acrodef{LTI}{linear and time-invariant}
\acrodef{FPGA}{field programmable gate array}
\acrodef{IRS}{intelligent reflective surface}
\acrodefplural{IRS}[IRS]{intelligent reflecting surfaces}
\acrodef{MIMO}{multiple-input multiple-output}
\acrodef{SISO}{single-input single-output}
\acrodef{QoS}{quality of service}
\acrodef{NOMA}{non-orthogonal multiple access}
\acrodef{SWIPT}{wireless information and power transfer}
\acrodef{EM}{electro magnetic}
\acrodef{HARQ}{hybrid automatic repeat request}
\acrodef{MCS}{modulation and coding scheme}
\acrodef{URLLC}{ultra-reliable low-latency communication}
\acrodef{PSDU}{physical layer service data unit}
\acrodef{PPDU}{physical layer protocol data unit}
\acrodef{PDU}{payload data unit}
\acrodef{MOS}{mean opinion score}
\acrodef{DMG}{directional multi-gigabit}
\acrodef{LDPC}{low-density parity-check}
\acrodef{FEC}{forward error correction}
\acrodef{PHY}{physical}
\acrodef{MAC}{medium access control}


%related to probability theory
\acrodef{PDF}{probability density function}
\acrodef{CDF}{cumulative density function}
\acrodef{PN}{Petri net}
\acrodef{MRSPN}{Markov regenerative stochastic Petri net}
\acrodef{MRGP}{Markov regenerative process}
\acrodef{MDP}{Markov decision process}


%related to ML
\acrodef{AI}{artificial intelligence}
\acrodef{ML}{machine learning}
\acrodef{RL}{reinforcement learning}
\acrodef{DRL}{deep reinforcement learning}
\acrodef{DQN}{deep Q-network}
\acrodef{PPO}{proximal policy optimization}
\acrodef{DBScan}{density-based spatial clustering}
\acrodef{NN}{neural network}
\acrodef{ANN}{artificial neural network}
\acrodef{RNN}{recurrent neural network}
\acrodef{CNN}{convolutional neural network}
\acrodef{LIME}{local interpretable model-agnostic explanations}
\acrodef{OMP}{group orthogonal matching pursuit}
\acrodef{ReLU}{rectified linear unit}
\acrodef{PDP}{partial dependence plot}
\acrodef{ICE}{individual conditional plot}

%related to optimization
\acrodef{SCA}{successive convex approximation}
\acrodef{BCD}{block coordinate descent}
\acrodef{GA}{genetic algorithm}
\acrodef{SDR}{semi-definite relaxation}
\acrodef{TS}{tabu search}
\acrodef{MM}{minimization-majorization}
\acrodef{GR}{Gaussian randomization}
\acrodef{LoS}{line-of-sight}

%related to detection and localization and synchronization
\acrodef{ToF}{time of flight}
\acrodef{AoA}{angle of arrival}
\acrodef{RSS}{received signal strength}
\acrodef{STO}{symbol time offset}
\acrodef{ROC}{receiver operating characteristic}
\acrodef{MAP}{maximum a posteriori}
